Programmable Spectrometry -- Per-pixel Classification of Materials using Learned Spectral Filters

Many materials have distinct spectral profiles. This facilitates estimation of the material composition of a scene at each pixel by first acquiring its hyperspectral image, and subsequently filtering it using a bank of spectral profiles. This process is inherently wasteful since only a set of linear projections of the acquired measurements contribute to the classification task. We propose a novel programmable camera that is capable of producing images of a scene with an arbitrary spectral filter. We use this camera to optically implement the spectral filtering of the scene's hyperspectral image with the bank of spectral profiles needed to perform per-pixel material classification. This provides gains both in terms of acquisition speed --- since only the relevant measurements are acquired --- and in signal-to-noise ratio --- since we invariably avoid narrowband filters that are light inefficient. Given training data, we use a range of classical and modern techniques including SVMs and neural networks to identify the bank of spectral profiles that facilitate material classification. We verify the method in simulations on standard datasets as well as real data using a lab prototype of the camera.

==> sup_introduction.tex <==
We presented a high spatial resolution, programmable spectral filter in the main paper. The key idea was to rely on a coded aperture to obtain invertible spatial and spectral blurs. By combining it with learned discriminating filters, we showed per-pixel classification results. 
%
The goal of the supplementary material:
\begin{enumerate}
	\item \emph{Theoretical background.} We present the image formation model for HSI that we used in our paper.
	
	\item \emph{Simulations.} We provided a brief result on simulations with the NASA Indian Pine dataset. We provide several more examples.
	
	\item \emph{Learning details.} We provide information about our neural network architecture with further details about system parameters.
	
	\item \emph{Details about lab prototype.} We provide details about our optical setup as well as steps on calibrating the system.
	
	%\item \emph{Real experiments.} We visualize some more experimental results and thoroughly quantify classification metrics. 
\end{enumerate}

==> sup_real.tex <==
\begin{figure*}[!tt]
	\centering
	\begin{subfigure}[c]{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/real/roc/roc3_rgb.jpg}
	\end{subfigure}
	\hspace{0.05em}
	\begin{subfigure}[c]{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/real/roc/roc4_rgb.png}
	\end{subfigure}
	\hspace{0.05em}
	\begin{subfigure}[c]{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/real/roc/roc5_rgb.png}
	\end{subfigure}
	\hspace{0.05em}
	\begin{subfigure}[c]{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/real/roc/roc6_rgb.png}
	\end{subfigure}
	\\
	\vspace{1em}
	\begin{subfigure}[c]{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/real/roc/roc3.pdf}
	\end{subfigure}
	\hspace{0.05em}
	\begin{subfigure}[c]{0.22\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/real/roc/roc4.pdf}
	\end{subfigure}
	\hspace{0.05em}
	\begin{subfigure}[c]{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/real/roc/roc5.pdf}
	\end{subfigure}
	\hspace{0.05em}
	\begin{subfigure}[c]{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/real/roc/roc6.pdf}
	\end{subfigure}
	\caption{\textbf{Performance of binary classifiers.} We show Receiver Operating Characteristic for four different scenarios here. Among various objects, ``wood" and ``fake wood" have lowest area under curve. Second, optically evaluating the linear projections leads to higher accuracy (red line) than capturing the cube completely and then classifying. Overall, our setup is capable of binary classification with high accuracy.}
	\label{fig:roc}
\end{figure*}

\paragraph{Receiver operating characteristic.}
%
Figure \ref{fig:roc} shows RoC curves for four scenes with binary classification. 

==> sup_simulations.tex <==
We showed simulations on the ``Indian Pine" dataset from NASA where the average accuracy was compared with state-of-art techniques in hyperspectral classification.
%
Our simulations showed that using spectral features alone reduced accuracy by a small amount but required far more measurements than the number of bands in the HSI.
%
We show simulations on some more datasets in comparison to state-of-art results along with visualization of labels in Fig.\ \ref{fig:sim}.
%
We used the same models for SVM and DNN as our real experiments.
%
To keep comparison fair between SVM and DNN, we set the number of spectral filters to number of object classes.
%
Overall, DNN outperforms SVM, often by a large margin.
%
More importantly, DNN is capable of achieving very high accuracy even when the first layer of the network is constrained to be linear, and fully connected.
%
This validates our hardware for classification tasks.

\begin{figure}[!tt]
	\centering
	\begin{subfigure}[t]{0.32\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sim/indian_pine/gt.png}
		\caption{Indian Pine}
	\end{subfigure}
	\hspace{0.01em}
	\begin{subfigure}[t]{0.32\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sim/indian_pine/svm.png}
		\caption{SVM ($83.1\%$)}
	\end{subfigure}
	\hspace{0.01em}
	\begin{subfigure}[t]{0.32\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sim/indian_pine/nn.png}
		\caption{DNN ($93.0\%$)}
	\end{subfigure}
	\\
	\begin{subfigure}[t]{0.32\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sim/pavia_center/gt.png}
		\caption{Pavia center}
	\end{subfigure}
	\hspace{0.01em}
	\begin{subfigure}[t]{0.32\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sim/pavia_center/svm.png}
		\caption{SVM ($96.5\%$)}
	\end{subfigure}
	\hspace{0.01em}
	\begin{subfigure}[t]{0.32\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sim/pavia_center/nn.png}
		\caption{DNN ($99.4\%$)}
	\end{subfigure}
	\\
	\begin{subfigure}[t]{0.32\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sim/pavia_univ/gt.png}
		\caption{Pavia center}
	\end{subfigure}
	\hspace{0.01em}
	\begin{subfigure}[t]{0.32\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sim/pavia_univ/svm.png}
		\caption{SVM ($82.2\%$)}
	\end{subfigure}
	\hspace{0.01em}
	\begin{subfigure}[t]{0.32\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sim/pavia_univ/nn.png}
		\caption{DNN ($96.7\%$)}
	\end{subfigure}
	\\
	\begin{subfigure}[t]{0.32\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sim/salinas/gt.png}
		\caption{Salinas}
	\end{subfigure}
	\hspace{0.01em}
	\begin{subfigure}[t]{0.32\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sim/salinas/svm.png}
		\caption{SVM ($91.6\%$)}
	\end{subfigure}
	\hspace{0.01em}
	\begin{subfigure}[t]{0.32\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sim/salinas/nn.png}
		\caption{DNN ($97.3\%$)}
	\end{subfigure}
	\caption{\small\textbf{Performance comparison.} Each dataset was trained with same number of spectral filters as number of object classes. Across the board, DNN has higher accuracy than SVM and can achieve near-perfect classification.}
	\label{fig:sim}
\end{figure}
